Odyssey: A Journey in the Land of Distributed Data Series Similarity Search

This paper presents Odyssey, a novel distributed data-series processing framework that efficiently addresses the critical challenges of exhibiting good speedup and ensuring high scalability in data series processing by taking advantage of the full computational capacity of modern clusters comprised of multi-core servers. Odyssey addresses a number of challenges in designing efficient and highly scalable distributed data series index, including efficient scheduling, and load-balancing without paying the prohibitive cost of moving data around. It also supports a flexible partial replication scheme, which enables Odyssey to navigate through a fundamental trade-off between data scalability and good performance during query answering. Through a wide range of configurations and using several real and synthetic datasets, our experimental analysis demonstrates that Odyssey achieves its challenging goals.

==> data-replication_ekosmas.tex <==
\lc{I have to rollback (or highlight any remaining of) my changes in this section.}

Odyssey aims at ensuring 
data scalability and, at the same time, good performance for query answering. 
Optimal data scalability requires to follow a no replication approach,
but experiments show that  the best query answering performance is noticed
for fully replicated settings. 
%
Odyssey manages to effectively navigate through
this trade-off between data scalability 
and good performance during query answering,
by providing a flexible {\it partial replication scheme}.
%which $partially$ replicates the dataset among the nodes. 
%that 
%enabling the development of $node-groups$. 
%This scheme 
%
Figure~\ref{fig:pdr_4_groups} schematically illustrates
how this scheme works in a system %of
with  $8$ nodes. 

%The idea is to split the set of nodes into a number of clusters, called {\em disjoint-partition clusters} such that 
%the nodes of a dijoint-partition cluster store a disjoint partition of the entire data series collection.
%Thus, the data sets stored in each node of a disjoint-partition cluster 
%are mutually disjoint and their union forms the entire data series collection. 
%%Figure~\ref{fig:pdr_2_groups} illustrates a configuration with 2 disjoint partition clusters
%%of 4 nodes each.
%Specifically, every 4 nodes of different color in the figure identify a cluster.  
The idea is to split the set of nodes into a number of clusters such that i) each node participates to 
exactly one cluster and ii) the set of data series stored in each node of a cluster are mutually disjoint 
(within the cluster), while their union forms the entire data series collection. 
%
%A {\em replication group} is a group of nodes such that each node stores the same data set as every other node in the group. 
%In Figure~\ref{fig:pdr_4_groups}, we have 4 replication groups. %, which are comprised of nodes [0-3] and [4-7], respectively.  
%%Similarly, Figure~\ref{fig:pdr_2_groups} illustrates 4 replication groups. 
%%In Figures \ref{fig:pdr_2_groups} and \ref{fig:pdr_4_groups} 
%The nodes of a 
%replication group are marked with the same color, whereas the nodes of
%a disjoint-partition cluster all have different colors. 
Additionally, a {\em replication group} is defined as the group of nodes that contain exactly the same set of data series.
Specifically, Figure~\ref{fig:pdr_4_groups} illustrates a configuration with $2$ clusters, each one having 
$4$ nodes (of different color), and $4$ replication groups, each one having $2$ nodes (of same color).
\lc{In Figure~\ref{fig:pdr_4_groups}, change the ``Disjoint-Partition Cluster'' with
``Clusters''. Also, we could update the figure so that nodes are presented exactly once, e.g. rows for replication groups
and columns for clusters.}
%
%The nodes of a replication group builds their iSAX indices from the same data. 
%%For example, in Figure~\ref{fig:pdr_2_groups}, 
%%each of the nodes[0-3] will build its index based on the first half of the dataset, 
%%whereas each of the nodes[4-7] will build an index based on the second half. 
%Thus, inside every replication group, we can apply the scheduling and load-balancing schemes,
%described in Sections~\ref{sched} and~\ref{load-balancing}, respectively. 
Since the nodes of a replication group build their iSAX indices using the same set of
data series, we can apply the scheduling and load-balancing schemes,
described in Sections~\ref{sched} and~\ref{load-balancing}, respectively. 

Notice that (for a fixed number of nodes) the number of clusters determines 
both the number of replication groups and the {\em replication degree} of the system.
In a configuration with $d$ clusters and $N$ nodes, each replication group
contains $N/d$ nodes and each node stores $d$ times more data than in the no-replication case.
%
%We experimented with replication groups of the same size, but 
%Odyssey can easily be adjusted to work for settings with replication groups of different sizes. 
%
%We define the {\em replication degree} of the system to be the number of
%disjoint-partition clusters it is comprised of. Replication degree $d$
%means that each node stores $d$ times more data than in the no-replication case. 
%In a system with $N$ nodes (where $N$ is a power of $2$), 
%Odyssey's data replication scheme supports $1, 2, 4, 8, \ldots, N$ clusters, 
%i.e. it supports $\Theta(\log N)$ different number of clusters.
%Smaller replication degrees 
Fewer clusters lead to smaller space overheads (and thus better data scalability). 
For example, %when the replication degree is $N$, 
in a configuration with $N$ clusters, all nodes store the entire data series collection,
whereas %a replication degree equal to $1$ 
using only a single cluster corresponds to the no-replication case, thus incurring no space overhead at all.
%Thus, Odyssey
Therefore, Odyssey's data replication scheme allows us to tackle memory limitation problems. 
%Moreover, more replication groups lead to scalability in index creation.

\lc{I suggest removing the definition of load factor.}
Additionally, fewer clusters lead to better index creation scalability.
To better understand this, 
%We 
we define the {\em load factor} to be the fraction 
of the number of nodes that share the same data %(i.e., the size of each replication group) 
divided by the total number of nodes in the system. 
This metric represents the percentage of the dataset that each node loads. 
For example, in full replication, %the size of a replication group 
the number of clusters is $N$ %(where $N$ is the number of system nodes), 
and the load factor is $1$, meaning that each individual node will load $100\%$ of the dataset.
 

We experimented with different %load factors 
number of clusters in %later sections 
Section~\ref{section:evaluation} to illustrate that
Odyssey nicely navigates through the discussed tradeoffs.
Specifically, considering a system with $N$ nodes (where $N$ is a power of $2$), 
Odyssey's data replication scheme supports $1, 2, 4, 8, \ldots, N$ clusters, 
i.e. $\Theta(\log N)$ different number of clusters, and replication groups of the 
same size. 
However, it can easily be adjusted to work for settings with any number of nodes
(not necessarily a power of $2$) and for replication groups of different sizes.
\lc{Is the last sentence correct?}


\remove{
\begin{figure}[tb]
	\centering
	\includegraphics[scale=0.26]{plots_chatzakis/theory/isax-two-groups-8-nodes-drawio.png}
	\caption{Partial Data Replication for a dataset of 80GB with two node groups.}
	\label{fig:pdr_2_groups}
\end{figure}
}
\begin{figure}[tb]
	\centering
	\includegraphics[scale=0.26]{plots_chatzakis/theory/isax-many-groups-8-nodes-drawio.png}
	\caption{Data Replication with four replication groups.}
	\label{fig:pdr_4_groups}
\end{figure}



%\here{Use terminology above in figures of this and later sections.}

\remove{
\begin{algorithm}[tb]
{
	\SetAlgoLined
	\KwIn{\textbf{Index} $index$, \textbf{Function} $exact\_search\_func$, \textbf{QuerySeries} $queries[]$, textbf{Integer} $queries\_size$, \textbf{Integer} $total\_nodes\_per\_nodegroup$}
	\vspace*{.1cm}
	\vspace*{.1cm}
	
	$node\_id \gets get\_node\_id()$;
	
	$query\_counter \gets 0$;
	
	\If{PREDICTIONS\_AVAILABLE} {$sort\_by\_predictions(queries)$;}
	
	\If{$node\_id$ is COORDINATOR of group}{
		<Send a query from $queries[]$ to the other nodes of the group and increments the $query\_counter$>;
	}

	\While{$(TRUE)$}{
		\If{$node\_id$ is COORDINATOR of group}{
		
		<Answer the requests of other nodes and increment $query\_counter$>;
		
		\If{$query\_counter \geq queries\_size$}{
			<Send $termination\_message$ to the nodes of the group>;
			
			break;
		}
		
		$exact\_search\_func(queries[query\_counter])$
		}
		\Else{
			$coordinator\_message \gets receive\_from\_group\_coordinator()$;
			
			\If{$coordinator\_message == termination\_message$}{break;}
			
			$query\_counter \gets coordinator\_message.query\_counter$
			
			$exact\_search\_func(queries[query\_counter])$
			
			<Request a new query from the group coordinator>;
		}
	}

	$workstealing\_helper()$;
	
}
\caption{Dynamic Distributed Query Answering with partial data $replication$}
\label{dynamic_query_answering}
\end{algorithm}

\begin{algorithm}[tb]
{
	\SetAlgoLined
	\KwIn{\textbf{QuerySeries} $queries[]$, \textbf{Integer} $total\_nodes\_per\_nodegroup$, $total\_queries$}
	\vspace*{.1cm}
	\vspace*{.1cm}
	
	$node\_id \gets get\_node\_id()$;
	
	$max\_score \gets 0$
	
	$coordinator\_id \gets group\_coord\_id(node\_id, total\_nodes\_per\_nodegroup)$;
	
	$current\_node\_id \gets coordinator\_id$;
	
	$node\_score \gets $ initialize with 0;
	
	\For{$q \gets 0$ \textbf{to} $total\_queries$}{
		$node\_score[current\_node\_id] += queries[q].prediction\_time$;
		
		<Node $current\_node\_id$ adds the query $q$ to its set>;
		
		\If{$node\_score[current\_node\_id] \geq max\_score$}{
			$max\_score \gets node\_score[current\_node\_id]$;
			
			$current\_node\_id \gets coordinator\_id + (current\_node\_id + 1) \mod total\_nodes\_per\_nodegroup$;
		}
	}
	

}
\caption{Greedy Query Scheduling using Predictions}
\label{static_query_answering}
\end{algorithm}
}




==> data-replication_ekosmas_with_diff.tex <==
\lc{I have to rollback (or highlight any remaining of) my changes in this section.}

Odyssey aims at ensuring 
data scalability and, at the same time, good performance for query answering. 
Optimal data scalability requires to follow a no replication approach,
but experiments show that  the best query answering performance is noticed
for fully replicated settings. 
%
Odyssey manages to effectively navigate through
this trade-off between data scalability 
and good performance during query answering,
by providing a flexible {\it partial replication scheme}.
%which $partially$ replicates the dataset among the nodes. 
%that 
%enabling the development of $node-groups$. 
%This scheme 
%
Figure~\ref{fig:pdr_4_groups} schematically illustrates
how this scheme works in a system %of
with  $8$ nodes. 
\lc{This last sentence was in the following paragraph.}


The idea is to split the set of nodes into a number of clusters\lsout{, called {\em disjoint-partition clusters} such that 
the nodes of a dijoint-partition cluster store a disjoint partition of the entire data series collection.
Thus, the data sets stored in each node of a disjoint-partition cluster 
are mutually disjoint and their union forms the entire data series collection.}
{such that i) each node participates to 
exactly one cluster and ii) the set of data series stored in each node of a cluster are mutually disjoint 
(within the cluster), while their union forms the entire data series collection.}
%Figure~\ref{fig:pdr_2_groups} illustrates a configuration with 2 disjoint partition clusters
%of 4 nodes each.
\lsout{Specifically, every 4 nodes of different color in the figure identify a cluster.}
%
%
{Additionally, a} %A 
{\em replication group} is \lsout{a group of nodes such that each node stores the same data set as every other node in the group.}
{defined as the group of nodes that contain exactly the same set of data series.}
{Specifically,} \lsout{In} Figure~\ref{fig:pdr_4_groups}, \lsout{we have 4 replication groups. %, which are comprised of nodes [0-3] and [4-7], respectively.  
%Similarly, Figure~\ref{fig:pdr_2_groups} illustrates 4 replication groups. 
%In Figures \ref{fig:pdr_2_groups} and \ref{fig:pdr_4_groups} 
The nodes of a 
replication group are marked with the same color, whereas the nodes of
a disjoint-partition cluster all have different colors. 
}
{illustrates a configuration with $2$ clusters, each one having 
$4$ nodes (of different color), and $4$ replication groups, each one having $2$ nodes (of same color).}
\lc{In Figure~\ref{fig:pdr_4_groups}, change the ``Disjoint-Partition Cluster'' with
``Clusters''. Also, we could update the figure so that nodes are presented exactly once, e.g. rows for replication groups
and columns for clusters.}
%
%
{Since the} \lsout{The} 
nodes of a replication group builds their iSAX indices \lsout{from} {using} the same {set of} 
data {series}\lsout{. 
%For example, in Figure~\ref{fig:pdr_2_groups}, 
%each of the nodes[0-3] will build its index based on the first half of the dataset, 
%whereas each of the nodes[4-7] will build an index based on the second half. 
Thus, inside every replication group,} we can apply the scheduling and load-balancing schemes,
described in Sections~\ref{sched} and~\ref{load-balancing}, respectively. 


{Notice that (for a fixed number of nodes) the number of clusters determines 
both the number of replication groups and the {\em replication degree} of the system.
In a configuration with $d$ clusters and $N$ nodes, each replication group
contains $N/d$ nodes and each node stores $d$ times more data than in the no-replication case.}
\lc{The following is moved at the end of the section, with the 2nd sentence be moved at the start
of this paragraph.}
\lsout{
We experimented with replication groups of the same size, but 
Odyssey can easily be adjusted to work for settings with replication groups of different sizes. 

We define the {\em replication degree} of the system to be the number of
disjoint-partition clusters it is comprised of. Replication degree $d$
means that each node stores $d$ times more data than in the no-replication case. 
In a system with $N$ nodes (where $N$ is a power of $2$), 
Odyssey's data replication scheme supports $1, 2, 4, 8, \ldots, N$ clusters, 
i.e. it supports $\Theta(\log N)$ different number of clusters.
}
\lsout{Smaller replication degrees} {Fewer clusters} lead to smaller space overheads (and thus better data scalability).
For example, \lsout{when the replication degree is $N$,}
{in a configuration with $N$ clusters}, all nodes store the entire data series collection,
whereas \lsout{a replication degree equal to $1$}
{using only a single cluster} corresponds to the no-replication case, thus incurring no space overhead at all.
\lsout{Thus, Odyssey}
{Therefore, Odyssey's} data replication scheme allows us to tackle memory limitation problems. 
\lsout{Moreover, more replication groups lead to scalability in index creation.}

\lc{I suggest removing the definition of load factor.}
{Additionally, fewer clusters lead to better index creation scalability.
To better understand this,}
\lsout{We}
we define the {\em load factor} to be the fraction 
of the number of nodes that share the same data \lsout{(i.e., the size of each replication group)}
divided by the total number of nodes in the system. 
This metric represents the percentage of the dataset that each node loads. 
For example, in full replication, \lsout{the size of a replication group}
the number of clusters is $N$ \lsout{(where $N$ is the number of system nodes),}
and the load factor is $1$, meaning that each individual node will load $100\%$ of the dataset.
 

We experimented with different \lsout{load factors}
{number of clusters} in \lsout{later sections }
{Section~\ref{section:evaluation}} to illustrate that
Odyssey nicely navigates through the discussed tradeoffs.
{Specifically, considering} a system with $N$ nodes (where $N$ is a power of $2$), 
Odyssey's data replication scheme supports $1, 2, 4, 8, \ldots, N$ clusters, 
i.e. it supports $\Theta(\log N)$ different number of clusters {and replication groups of the 
same size. 
However, it can easily be adjusted to work for settings with any number of nodes
(not necessarily a power of $2$) and for replication groups of different sizes.}
\lc{Is the last sentence correct?}


\remove{
\begin{figure}[tb]
	\centering
	\includegraphics[scale=0.26]{plots_chatzakis/theory/isax-two-groups-8-nodes-drawio.png}
	\caption{Partial Data Replication for a dataset of 80GB with two node groups.}
	\label{fig:pdr_2_groups}
\end{figure}
}
\begin{figure}[tb]
	\centering
	\includegraphics[scale=0.26]{plots_chatzakis/theory/isax-many-groups-8-nodes-drawio.png}
	\caption{Data Replication with four replication groups.}
	\label{fig:pdr_4_groups}
\end{figure}



%\here{Use terminology above in figures of this and later sections.}

\remove{
\begin{algorithm}[tb]
{
	\SetAlgoLined
	\KwIn{\textbf{Index} $index$, \textbf{Function} $exact\_search\_func$, \textbf{QuerySeries} $queries[]$, textbf{Integer} $queries\_size$, \textbf{Integer} $total\_nodes\_per\_nodegroup$}
	\vspace*{.1cm}
	\vspace*{.1cm}
	
	$node\_id \gets get\_node\_id()$;
	
	$query\_counter \gets 0$;
	
	\If{PREDICTIONS\_AVAILABLE} {$sort\_by\_predictions(queries)$;}
	
	\If{$node\_id$ is COORDINATOR of group}{
		<Send a query from $queries[]$ to the other nodes of the group and increments the $query\_counter$>;
	}

	\While{$(TRUE)$}{
		\If{$node\_id$ is COORDINATOR of group}{
		
		<Answer the requests of other nodes and increment $query\_counter$>;
		
		\If{$query\_counter \geq queries\_size$}{
			<Send $termination\_message$ to the nodes of the group>;
			
			break;
		}
		
		$exact\_search\_func(queries[query\_counter])$
		}
		\Else{
			$coordinator\_message \gets receive\_from\_group\_coordinator()$;
			
			\If{$coordinator\_message == termination\_message$}{break;}
			
			$query\_counter \gets coordinator\_message.query\_counter$
			
			$exact\_search\_func(queries[query\_counter])$
			
			<Request a new query from the group coordinator>;
		}
	}

	$workstealing\_helper()$;
	
}
\caption{Dynamic Distributed Query Answering with partial data $replication$}
\label{dynamic_query_answering}
\end{algorithm}

\begin{algorithm}[tb]
{
	\SetAlgoLined
	\KwIn{\textbf{QuerySeries} $queries[]$, \textbf{Integer} $total\_nodes\_per\_nodegroup$, $total\_queries$}
	\vspace*{.1cm}
	\vspace*{.1cm}
	
	$node\_id \gets get\_node\_id()$;
	
	$max\_score \gets 0$
	
	$coordinator\_id \gets group\_coord\_id(node\_id, total\_nodes\_per\_nodegroup)$;
	
	$current\_node\_id \gets coordinator\_id$;
	
	$node\_score \gets $ initialize with 0;
	
	\For{$q \gets 0$ \textbf{to} $total\_queries$}{
		$node\_score[current\_node\_id] += queries[q].prediction\_time$;
		
		<Node $current\_node\_id$ adds the query $q$ to its set>;
		
		\If{$node\_score[current\_node\_id] \geq max\_score$}{
			$max\_score \gets node\_score[current\_node\_id]$;
			
			$current\_node\_id \gets coordinator\_id + (current\_node\_id + 1) \mod total\_nodes\_per\_nodegroup$;
		}
	}
	

}
\caption{Greedy Query Scheduling using Predictions}
\label{static_query_answering}
\end{algorithm}
}



